Search for Efficient Large Language Models

Large Language Models (LLMs) have long held sway in the realms of artificial intelligence research. Numerous efficient techniques, including weight pruning, quantization, and distillation, have been embraced to compress LLMs, targeting memory reduction and inference acceleration, which underscore the redundancy in LLMs. However, most model compression techniques concentrate on weight optimization, overlooking the exploration of optimal architectures. Besides, traditional architecture search methods, limited by the elevated complexity with extensive parameters, struggle to demonstrate their effectiveness on LLMs. In this paper, we propose a training-free architecture search framework to identify optimal subnets that preserve the fundamental strengths of the original LLMs while achieving inference acceleration. Furthermore, after generating subnets that inherit specific weights from the original LLMs, we introduce a reformation algorithm that utilizes the omitted weights to rectify the inherited weights with a small amount of calibration data. Compared with SOTA training-free structured pruning works that can generate smaller networks, our method demonstrates superior performance across standard benchmarks. Furthermore, our generated subnets can directly reduce the usage of GPU memory and achieve inference acceleration. Code: https://github.com/shawnricecake/search-llm

==> algorithms/search_process.tex <==


% \begin{algorithm}
% \caption{Search Process} % Caption for the algorithm
% \label{alg:search_process}

% \begin{algorithmic}[0] % The number tells where the line numbering should start

% % \Function{\bfseries mutate}{subnet $\mathcal{F}_x=[f_x^1(Q_x^1), f_x^2,..,f_x^n]$, mutation spaces $\mathcal{Q}$, depth probability $p_d$, mutate probability $p_m$}

% %     $p = random[0, 1]$
% %     \If{$p > p_d$}  % If statement
    
% %     $d_{new} = random ( \mathcal{Q}[depth] )$
    
% %     $\mathcal{F}_x = \mathcal{F}_x[:d_{new}]$
    
% %     \EndIf

% %     \For{$i_{th}$ layer $f_x^i$ in $\mathcal{F}_x$} % space for loop

    
    
% %         \For{mutation space $q_y$ \textbf{in} $\mathcal{Q}$} % space for loop
        
% %         \If{$q_y == depth$}  % If statement
% %         \textbf{continue} 
% %         \EndIf

% %         $p = random[0, 1]$
% %         \If{$p > p_m$}
        
        
% %         \EndIf
        
    
% %         \EndFor
    
% %     \EndFor
    
% %     \State \textbf{return} $result$
% % \EndFunction

% \State {\bfseries input:} training epochs $T$, train dataset $\mathbf{D}_{train}$, original model $\mathcal{F}$, initial selection masks $\mathcal{S}^*_0$, mutation space $\mathcal{Q}$, number of generate $\alpha$, probability of generate $p_g$, number of mutation $\beta$, probability of mutation $p_m$.

% % \State {\bfseries initialization:} $ \mathcal{S}^* \gets $ Eq~\ref{eq:initialize_select_mask} 

% % \State {\bfseries generate:} 
% \Procedure{generate}{}
%     \For{$i$ \textbf{in} $1$ \textbf{to} $\alpha$}
%     $ \mathcal{G} \gets add \    mutate[ \mathcal{F} , \mathcal{S}^*_0 , p_g ] $ 
%     \EndFor
% \EndProcedure, \ $ \mathcal{G} = \{ \mathcal{S}_i \}_{i=1}^{\alpha} $

% % \State {\bfseries evaluate \& update top-100:} $ \mathcal{A} \gets \{ \mathcal{S}_i^* \}_{i=1}^{100} = {top}_{100} [evaluate( \{ \mathcal{S}_i \}_{i =1}^{\alpha}, \mathbf{D}_{train} )] $
% \Procedure{evaluate \& update top-100}{}
%     \For{$i$ \textbf{in} $1$ \textbf{to} $\alpha$}
%     {
%      $ \mathcal{A} \gets update \   {top}_{100} [evaluate(  \mathcal{S}_i , \mathbf{D}_{train} )] $
%      }
%     % \EndFor
% \EndProcedure, \ $ \mathcal{A} = \{ \mathcal{S}_i^* \}_{i=1}^{100} $


% \For{$i$ \textbf{in} $1$ \textbf{to} $T$} % epoch for loop
%     % \State {\bfseries mutation:}  $ \{ \mathcal{S}_i \}_{i =1}^{\beta} =    mutate[\mathcal{F},  random( \mathcal{A}) , p_m ]  $
%     \Procedure{mutation}{}
%     \For{$i$ \textbf{in} $1$ \textbf{to} $\alpha$}
%      $ \mathcal{M} \gets add \    mutate[ \mathcal{F} , random( \mathcal{A}) , p_m ] $ 
%     \EndFor
%     \EndProcedure, \ $ \mathcal{M} = \{ \mathcal{S}_i \}_{i=1}^{\beta} $

%     % \State {\bfseries regenerate:} $ \{ \mathcal{S}_i \}_{i=1}^{\alpha} =    mutate(\mathcal{F} , \mathcal{S}^*_0 , p_g ) $ 
%     \Procedure{regenerate}{}
%     \For{$i$ \textbf{in} $1$ \textbf{to} $\alpha$}
%      $ \mathcal{G} \gets add \    mutate[\mathcal{F} , \mathcal{S}^*_0 , p_g ] $ 
%     \EndFor
%     \EndProcedure, \ $ \mathcal{G} = \{ \mathcal{S}_i \}_{i=1}^{\alpha} $

%     % \State {\bfseries evaluate \& update top-100:} $ \mathcal{A} \gets 
%     % \{ \mathcal{S}_i^* \}_{i=1}^{100} = 
%     % {top}_{100} [evaluate( \{ \mathcal{S}_i \}_{i =1}^{\alpha} \cup \{ \mathcal{S}_i \}_{i =1}^{\beta}, \mathbf{D}_{train} )] $
%     \Procedure{evaluate \& update top-100}{}
%     \For{$\mathcal{S}_i$ \textbf{in} $\mathcal{G} \cup \mathcal{M}$}
%      $ \mathcal{A} \gets update \   {top}_{100} [evaluate(  \mathcal{S}_i , \mathbf{D}_{train} )] $ 
%     \EndFor
%     \EndProcedure, \ $ \mathcal{A} = \{ \mathcal{S}_i^* \}_{i=1}^{100} $

    
% \EndFor
% \State \textbf{return} $\mathcal{A}$ % Return statement

% \end{algorithmic}
% \end{algorithm}


\begin{wrapfigure}{R}{0.56\textwidth}
\begin{algorithm}[H]
% \SetAlgoNoLine  
        \label{alg:search_process}
        \caption{Search Process}
        \KwIn{
        training epochs $T$, train dataset $\mathbf{D}_{train}$, original model $\mathcal{F}$, initial selection masks $\mathcal{S}^*_0$, mutation space $\mathcal{Q}$, number of generate $\alpha$, probability of generate $p_g$, number of mutation $\beta$, probability of mutation $p_m$.
        }
        % \KwOut{
        % optimal subnets $\mathcal{A}$
        % }
        
        \tcp{Initialize with $\mathcal{S}^*_0$ : }

        % \begin{minipage}{0.5\linewidth}
        \For{$i$ \textbf{in} $1$ \textbf{to} $\alpha$}
        {
        $ \mathcal{G} \gets add \    mutate[ \mathcal{F} , \mathcal{S}^*_0 , p_g ] $ 
        }
        % \end{minipage}


        \tcp{Evaluate \& Update $\mathcal{A}$:}
        \For{$i$ \textbf{in} $1$ \textbf{to} $\alpha$}
        {
         $ \mathcal{A} \gets update \   {top}_{100} [evaluate(  \mathcal{S}_i , \mathbf{D}_{train} )] $
         }


        \tcp{Evolution:}
        \For{$i$ \textbf{in} $1$ \textbf{to} $T$}{
        % \State {\bfseries mutation:}  $ \{ \mathcal{S}_i \}_{i =1}^{\beta} =    mutate[\mathcal{F},  random( \mathcal{A}) , p_m ]  $
        \tcp{Mutation:}
        \For{$i$ \textbf{in} $1$ \textbf{to} $\alpha$}{
         $ \mathcal{M} \gets add \    mutate[ \mathcal{F} , random( \mathcal{A}) , p_m ] $ 
        }
        % $ \mathcal{M} = \{ \mathcal{S}_i \}_{i=1}^{\beta} $
    
        \tcp{Regenerate:}
        \For{$i$ \textbf{in} $1$ \textbf{to} $\alpha$}{
         $ \mathcal{G} \gets add \    mutate[\mathcal{F} , \mathcal{S}^*_0 , p_g ] $ 
        }
        % $ \mathcal{G} = \{ \mathcal{S}_i \}_{i=1}^{\alpha} $
    
        \tcp{Evaluate \& Update $\mathcal{A}$:}
        \For{$\mathcal{S}_i$ \textbf{in} $\mathcal{G} \cup \mathcal{M}$}{
        
         $ \mathcal{A} \gets update \   {top}_{100} [evaluate(  \mathcal{S}_i , \mathbf{D}_{train} )] $ 
        }
        % $ \mathcal{A} = \{ \mathcal{S}_i^* \}_{i=1}^{100} $
        }
        
        \KwOut{
        optimal subnets $\mathcal{A}$
        }

\end{algorithm}
\end{wrapfigure}

==> sections/7_checklist.tex <==
\section*{NeurIPS Paper Checklist}

% %%% BEGIN INSTRUCTIONS %%%
% The checklist is designed to encourage best practices for responsible machine learning research, addressing issues of reproducibility, transparency, research ethics, and societal impact. Do not remove the checklist: {\bf The papers not including the checklist will be desk rejected.} The checklist should follow the references and follow the (optional) supplemental material.  The checklist does NOT count towards the page
% limit. 

% Please read the checklist guidelines carefully for information on how to answer these questions. For each question in the checklist:
% \begin{itemize}
%     \item You should answer \answerYes{}, \answerNo{}, or \answerNA{}.
%     \item \answerNA{} means either that the question is Not Applicable for that particular paper or the relevant information is Not Available.
%     \item Please provide a short (1–2 sentence) justification right after your answer (even for NA). 
%    % \item {\bf The papers not including the checklist will be desk rejected.}
% \end{itemize}

% {\bf The checklist answers are an integral part of your paper submission.} They are visible to the reviewers, area chairs, senior area chairs, and ethics reviewers. You will be asked to also include it (after eventual revisions) with the final version of your paper, and its final version will be published with the paper.

% The reviewers of your paper will be asked to use the checklist as one of the factors in their evaluation. While "\answerYes{}" is generally preferable to "\answerNo{}", it is perfectly acceptable to answer "\answerNo{}" provided a proper justification is given (e.g., "error bars are not reported because it would be too computationally expensive" or "we were unable to find the license for the dataset we used"). In general, answering "\answerNo{}" or "\answerNA{}" is not grounds for rejection. While the questions are phrased in a binary way, we acknowledge that the true answer is often more nuanced, so please just use your best judgment and write a justification to elaborate. All supporting evidence can appear either in the main paper or the supplemental material, provided in appendix. If you answer \answerYes{} to a question, in the justification please point to the section(s) where related material for the question can be found.

% IMPORTANT, please:
% \begin{itemize}
%     \item {\bf Delete this instruction block, but keep the section heading ``NeurIPS paper checklist"},
%     \item  {\bf Keep the checklist subsection headings, questions/answers and guidelines below.}
%     \item {\bf Do not modify the questions and only use the provided macros for your answers}.
% \end{itemize} 
 

% %%% END INSTRUCTIONS %%%


\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We explain method and summarize the contribution in introduction.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the abstract and introduction do not include the claims made in the paper.
        \item The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations. A No or NA answer to this question will not be perceived well by the reviewers. 
        \item The claims made should match theoretical and experimental results, and reflect how much the results can be expected to generalize to other settings. 
        \item It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper. 
    \end{itemize}

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The limitation is included in conclusion section.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper has no limitation while the answer No means that the paper has limitations, but those are not discussed in the paper. 
        \item The authors are encouraged to create a separate "Limitations" section in their paper.
        \item The paper should point out any strong assumptions and how robust the results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only holding locally). The authors should reflect on how these assumptions might be violated in practice and what the implications would be.
        \item The authors should reflect on the scope of the claims made, e.g., if the approach was only tested on a few datasets or with a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated.
        \item The authors should reflect on the factors that influence the performance of the approach. For example, a facial recognition algorithm may perform poorly when image resolution is low or images are taken in low lighting. Or a speech-to-text system might not be used reliably to provide closed captions for online lectures because it fails to handle technical jargon.
        \item The authors should discuss the computational efficiency of the proposed algorithms and how they scale with dataset size.
        \item If applicable, the authors should discuss possible limitations of their approach to address problems of privacy and fairness.
        \item While the authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection, a worse outcome might be that reviewers discover limitations that aren't acknowledged in the paper. The authors should use their best judgment and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed to not penalize honesty concerning limitations.
    \end{itemize}

\item {\bf Theory Assumptions and Proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We provide the theorem in methodology section and the proof in appendix.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include theoretical results. 
        \item All the theorems, formulas, and proofs in the paper should be numbered and cross-referenced.
        \item All assumptions should be clearly stated or referenced in the statement of any theorems.
        \item The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, the authors are encouraged to provide a short proof sketch to provide intuition. 
        \item Inversely, any informal proof provided in the core of the paper should be complemented by formal proofs provided in appendix or supplemental material.
        \item Theorems and Lemmas that the proof relies upon should be properly referenced. 
    \end{itemize}

    \item {\bf Experimental Result Reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We provide the detailed experiment setup in experiment section.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item If the paper includes experiments, a No answer to this question will not be perceived well by the reviewers: Making the paper reproducible is important, regardless of whether the code and data are provided or not.
        \item If the contribution is a dataset and/or model, the authors should describe the steps taken to make their results reproducible or verifiable. 
        \item Depending on the contribution, reproducibility can be accomplished in various ways. For example, if the contribution is a novel architecture, describing the architecture fully might suffice, or if the contribution is a specific model and empirical evaluation, it may be necessary to either make it possible for others to replicate the model with the same dataset, or provide access to the model. In general. releasing code and data is often one good way to accomplish this, but reproducibility can also be provided via detailed instructions for how to replicate the results, access to a hosted model (e.g., in the case of a large language model), releasing of a model checkpoint, or other means that are appropriate to the research performed.
        \item While NeurIPS does not require releasing code, the conference does require all submissions to provide some reasonable avenue for reproducibility, which may depend on the nature of the contribution. For example
        \begin{enumerate}
            \item If the contribution is primarily a new algorithm, the paper should make it clear how to reproduce that algorithm.
            \item If the contribution is primarily a new model architecture, the paper should describe the architecture clearly and fully.
            \item If the contribution is a new model (e.g., a large language model), then there should either be a way to access this model for reproducing the results or a way to reproduce the model (e.g., with an open-source dataset or instructions for how to construct the dataset).
            \item We recognize that reproducibility may be tricky in some cases, in which case authors are welcome to describe the particular way they provide for reproducibility. In the case of closed-source models, it may be that access to the model is limited in some way (e.g., to registered users), but it should be possible for other researchers to have some path to reproducing or verifying the results.
        \end{enumerate}
    \end{itemize}


\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The dataset and model we used is open-source.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that paper does not include experiments requiring code.
        \item Please see the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item While we encourage the release of code and data, we understand that this might not be possible, so “No” is an acceptable answer. Papers cannot be rejected simply for not including code, unless this is central to the contribution (e.g., for a new open-source benchmark).
        \item The instructions should contain the exact command and environment needed to run to reproduce the results. See the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item The authors should provide instructions on data access and preparation, including how to access the raw data, preprocessed data, intermediate data, and generated data, etc.
        \item The authors should provide scripts to reproduce all experimental results for the new proposed method and baselines. If only a subset of experiments are reproducible, they should state which ones are omitted from the script and why.
        \item At submission time, to preserve anonymity, the authors should release anonymized versions (if applicable).
        \item Providing as much information as possible in supplemental material (appended to the paper) is recommended, but including URLs to data and code is permitted.
    \end{itemize}


\item {\bf Experimental Setting/Details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer, etc.) necessary to understand the results?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We provide detailed experiment setting in experiment section.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The experimental setting should be presented in the core of the paper to a level of detail that is necessary to appreciate the results and make sense of them.
        \item The full details can be provided either with the code, in appendix, or as supplemental material.
    \end{itemize}

\item {\bf Experiment Statistical Significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We did not report error bars.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The authors should answer "Yes" if the results are accompanied by error bars, confidence intervals, or statistical significance tests, at least for the experiments that support the main claims of the paper.
        \item The factors of variability that the error bars are capturing should be clearly stated (for example, train/test split, initialization, random drawing of some parameter, or overall run with given experimental conditions).
        \item The method for calculating the error bars should be explained (closed form formula, call to a library function, bootstrap, etc.)
        \item The assumptions made should be given (e.g., Normally distributed errors).
        \item It should be clear whether the error bar is the standard deviation or the standard error of the mean.
        \item It is OK to report 1-sigma error bars, but one should state it. The authors should preferably report a 2-sigma error bar than state that they have a 96\% CI, if the hypothesis of Normality of errors is not verified.
        \item For asymmetric distributions, the authors should be careful not to show in tables or figures symmetric error bars that would yield results that are out of range (e.g. negative error rates).
        \item If error bars are reported in tables or plots, The authors should explain in the text how they were calculated and reference the corresponding figures or tables in the text.
    \end{itemize}

\item {\bf Experiments Compute Resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We explain the computation resources in experiment section.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The paper should indicate the type of compute workers CPU or GPU, internal cluster, or cloud provider, including relevant memory and storage.
        \item The paper should provide the amount of compute required for each of the individual experimental runs as well as estimate the total compute. 
        \item The paper should disclose whether the full research project required more compute than the experiments reported in the paper (e.g., preliminary or failed experiments that didn't make it into the paper). 
    \end{itemize}
    
\item {\bf Code Of Ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Research is conducted in the paper conform with NeurIPS Code of Ethics.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the authors have not reviewed the NeurIPS Code of Ethics.
        \item If the authors answer No, they should explain the special circumstances that require a deviation from the Code of Ethics.
        \item The authors should make sure to preserve anonymity (e.g., if there is a special consideration due to laws or regulations in their jurisdiction).
    \end{itemize}


\item {\bf Broader Impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We discuss them in conclusion.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that there is no societal impact of the work performed.
        \item If the authors answer NA or No, they should explain why their work has no societal impact or why the paper does not address societal impact.
        \item Examples of negative societal impacts include potential malicious or unintended uses (e.g., disinformation, generating fake profiles, surveillance), fairness considerations (e.g., deployment of technologies that could make decisions that unfairly impact specific groups), privacy considerations, and security considerations.
        \item The conference expects that many papers will be foundational research and not tied to particular applications, let alone deployments. However, if there is a direct path to any negative applications, the authors should point it out. For example, it is legitimate to point out that an improvement in the quality of generative models could be used to generate deepfakes for disinformation. On the other hand, it is not needed to point out that a generic algorithm for optimizing neural networks could enable people to train models that generate Deepfakes faster.
        \item The authors should consider possible harms that could arise when the technology is being used as intended and functioning correctly, harms that could arise when the technology is being used as intended but gives incorrect results, and harms following from (intentional or unintentional) misuse of the technology.
        \item If there are negative societal impacts, the authors could also discuss possible mitigation strategies (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of ML).
    \end{itemize}
    
\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pretrained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We discussed in introduction.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper poses no such risks.
        \item Released models that have a high risk for misuse or dual-use should be released with necessary safeguards to allow for controlled use of the model, for example by requiring that users adhere to usage guidelines or restrictions to access the model or implementing safety filters. 
        \item Datasets that have been scraped from the Internet could pose safety risks. The authors should describe how they avoided releasing unsafe images.
        \item We recognize that providing effective safeguards is challenging, and many papers do not require this, but we encourage authors to take this into account and make a best faith effort.
    \end{itemize}

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We originally implemented our method.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not use existing assets.
        \item The authors should cite the original paper that produced the code package or dataset.
        \item The authors should state which version of the asset is used and, if possible, include a URL.
        \item The name of the license (e.g., CC-BY 4.0) should be included for each asset.
        \item For scraped data from a particular source (e.g., website), the copyright and terms of service of that source should be provided.
        \item If assets are released, the license, copyright information, and terms of use in the package should be provided. For popular datasets, \url{paperswithcode.com/datasets} has curated licenses for some datasets. Their licensing guide can help determine the license of a dataset.
        \item For existing datasets that are re-packaged, both the original license and the license of the derived asset (if it has changed) should be provided.
        \item If this information is not available online, the authors are encouraged to reach out to the asset's creators.
    \end{itemize}

\item {\bf New Assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We introduced in the introduction.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not release new assets.
        \item Researchers should communicate the details of the dataset/code/model as part of their submissions via structured templates. This includes details about training, license, limitations, etc. 
        \item The paper should discuss whether and how consent was obtained from people whose asset is used.
        \item At submission time, remember to anonymize your assets (if applicable). You can either create an anonymized URL or include an anonymized zip file.
    \end{itemize}

\item {\bf Crowdsourcing and Research with Human Subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: There is nothing related to human subjects in our work.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Including this information in the supplemental material is fine, but if the main contribution of the paper involves human subjects, then as much detail as possible should be included in the main paper. 
        \item According to the NeurIPS Code of Ethics, workers involved in data collection, curation, or other labor should be paid at least the minimum wage in the country of the data collector. 
    \end{itemize}

\item {\bf Institutional Review Board (IRB) Approvals or Equivalent for Research with Human Subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: There is nothing related to human subjects in our work.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Depending on the country in which research is conducted, IRB approval (or equivalent) may be required for any human subjects research. If you obtained IRB approval, you should clearly state this in the paper. 
        \item We recognize that the procedures for this may vary significantly between institutions and locations, and we expect authors to adhere to the NeurIPS Code of Ethics and the guidelines for their institution. 
        \item For initial submissions, do not include any information that would break anonymity (if applicable), such as the institution conducting the review.
    \end{itemize}

\end{enumerate}


==> sections/8_rebuttal.tex <==

\textcolor{blue}{Global Response}

We would like to thank the reviewers for their positive comments and constructive feedback on our paper. We sincerely appreciate the reviewers for acknowledging that our work overcomes the limitations of prior research and would benefit the community (Reviewer Xurt, BSTA). We are pleased that our method is considered novel, useful, clear, reasonable, general, and high-performing without requiring additional training (Reviewer n31G, Qp2U, Xurt, BSTA). Additionally, we are grateful for the recognition of our comprehensive and impressive experiments and results (Reviewer Xurt), as well as the clarity and quality of our writing (Reviewer Qp2U, Xurt). 

We have devoted substantial efforts to address all the reviewers' questions and to enhance our experiments during the rebuttal phase. Detailed responses to each reviewer are provided below.

\textbf{Search Cost}

We can reduce our search cost with similar performance. 
For the search cost, it usually takes only 20 epochs for the convergence, and more epochs beyond 20 lead to marginal improvements (see Figure 5). For LLaMA-7B, we run 50 epochs (5 hours) for better results. When searching for 20 epochs, the perplexity for LLaMA-7B with 10\% and 20\% sparsity on WikiText2 are 6.23 and 7.21, which are still better than all baselines in Table 2. Besides, for large models such as LLaMA-65B, we only adopt 20 epochs for faster search, which takes 5 hours. 

Besides, we highlight that our search cost is just similar to the baselines.

For LLM-Pruner, it is very difficult to scale to larger models such as LLaMA-30B and LLaMA-65B, as it requires the backward propagation to compute the gradients for identifying the weight importance, incurring much larger memory and complexity cost. It only has the results for 7B models (such as LLaMA-7B, and Vicuna-7B) and LLaMA-13B. The 7B models require 3 hours to finish the compression. 

For SliceGPT, it requires 5 hours to finish the pruning and fine-tuning of LLaMA-2 70B, which is similar to ours with 5 hours of search for LLaMA-65B. SliceGPT relies on PCA (Principal Component Analysis) to identify and remove less significant weights, which computes the eigenvectors and eigenvalues of the covariance matrix of the signal matrix. For large models, this step is computationally demanding and time-consuming because it requires processing a substantial amount of data to compute these matrices accurately. Besides, this work notes that using double precision for eigenvector calculations in PCA is necessary to avoid numerical errors that can degrade performance. This choice further increases the computational load and time required for pruning. It is data hungry and requires to use much more calibration samples (1024) while our method only uses 128 samples.




\textbf{Mask Sharing}

As discussed in Line 124-128, the model has multiple blocks (i.e., layers of LLaMA model). Each block has two modules, the self-attention module and MLP module. Each module contains multiple weights, such as the query, key, value in the self-attention module and up, gate, down in MLP module (Line 124-128). Mask sharing means that different weights in the same module share the same mask. However, modules of different blocks do not necessarily share the same mask. Each block has two masks corresponding to its self-attention module and MLP module, respectively. Different blocks do not share masks, and they have their own masks, which are not necessarily the same. Just as Reviewer BTSA mentioned, Figure 2 middle shows that different blocks can have different masks/sparsity.

Initially, different masks have the same inheriting ratios. But the masks can still be different although their sparsity are the same. After we begin our search, the inheriting ratios of different masks can be different, although they start from the same value.




\textbf{Additional Results}

We further provide more results with lower inheriting ratios and fine-tuning in Table 8 as follows,

%------------Table 8 markdown --------------------------
% Table 8
% | Method           | Inheriting Ratio | Wiki PPL↓ | PTB PPL↓ | BoolQ | PIQA | HellaSwag | WinoGrande | ARC-e | ARC-c | OBQA | Average Acc.↑ |
% |------------------|------------------|-----------|----------|-------|------|-----------|------------|-------|-------|------|----------------|
% | LLM-Pruner       | 80%              | 11.97     | 55.68    | 59.39 | 75.57| 65.34     | 61.33      | 59.18 | 37.12 | 39.80| 56.82          |
% | LLM-Pruner (LoRA)| 80%              | 8.41      | 41.78    | 67.78 | 76.36| 68.14     | 64.32      | 63.41 | 36.87 | 40.10| 59.57          |
% | Ours             | 80%              | **6.89**  | **36.06**| 70.98 | 74.92| 67.29     | 64.64      | 64.23 | 36.52 | 39.40| **59.71**      |
% | Ours (LoRA)      | 80%              | 6.57      | 34.32    | 71.19 | 75.01| 68.43     | 64.12      | 63.88 | 35.44 | 40.03| 59.73          |
% | LLM-Pruner       | 50%              | 126.02    | 460.71   | 51.97 | 60.23| 35.89     | 49.07      | 32.76 | 25.67 | 34.91| 41.50          |
% | LLM-Pruner (LoRA)| 50%              | 51.56     | 198.76   | 60.98 | 69.12| 47.83     | 55.78      | 46.92 | 28.56 | 35.64| 49.26          |
% | Ours             | 50%              | **15.48** | **117.06**| 61.27 | 69.13| 51.18     | 57.78      | 52.16 | 29.34 | 35.45| **50.79**      |
% | Ours (LoRA)      | 80%              | 11.34     | 83.48    | 63.49 | 73.03| 56.93     | 59.21      | 48.87 | 36.12 | 36.23| 53.41          |
%------------Table 8 markdown --------------------------







\textcolor{blue}{Response to Reviewer n31g}


\textbf{Weakness 1. Difference from network pruning}

Our proposed search method significantly differs from standard neural network pruning techniques. Specifically, our method includes a search initialization process to identify the effective initial architecture and an evolution architecture search with special mask mutation and efficient candidate evaluation, which are not typical in standard weight pruning techniques. We are the first to incorporate the architecture search technique for LLMs to find efficient architectures. There are no other search baselines and thus we mainly compare with pruning works. Although our method significantly differs from traditional pruning, both our search and pruning can lead to efficient lightweight LLMs. 




\textbf{Weakness 2. Reformation}

Thanks for the suggestion, we will explain more about the reformation in the abstract and introduction.


\textbf{Weakness 3. Search cost}

% pu:
% We highlight that our search cost is just similar to the baselines. For example, as discussed in their original papers, LLM-Pruner requires 3 hours for the compression of LLaMA-7B. For SliceGPT, all LLaMA-2, OPT and Phi-2 models can be sliced in 1 to 3 hours. With recovery fine-tuning, it compresses all LLMs in 1 to 5 hours in total. Our method takes 5 hours for 50 epochs for LLaMA-7B during the search on one single GPU. We can see that our search cost is similar to the baselines. Compared with traditional architecture search method requiring days or weeks of training, our search cost is minor, which is achieved through our efficiency designs such as  effective initialization and quick candidate evaluation, demonstrated in Figure 5.

We highlight that our search cost is just similar to the baselines. Details can be found in the above global rebuttal.


\textbf{Weakness 3.a Performance as a function of search cost.}

% pu:
% Furthermore, we can reduce the search cost without significantly sacrificing the performance. Our method is trained with 50 epochs for 5 hours. Figure 5 clearly demonstrates how the proposed method performs as a function of the search budget (number of epochs and thus search hours). As shown in our Figure 5 for convergence analysis, our method converges at 20 epochs, and more epochs do not result in significant improvements. We can reduce our search cost by only training 20 epochs, which just takes about 2 hours. Note that with 20 epochs, for LLaMA-7B, we can still achieve  6.23 and 7.21 perplexity on WikiText2 under 90\% and 80\% inheriting ratios, respectively, which are better than all baselines shown in Table 2. We can still perform better with reduced search cost. Besides, for large models such as LLaMA-65B, we only adopt 20 epochs for faster search, which takes 5 hours. 

Figure 5 clearly demonstrates how the proposed method performs as a function of the search budget (number of epochs and thus search hours).
As we discussed in the global rebuttal, we can reduce the search cost without significantly sacrificing the performance.
Note that, with 20 epochs, for LLaMA-7B, we can still achieve  6.23 and 7.21 perplexity on WikiText2 under 90\% and 80\% inheriting ratios, respectively, which are better than all baselines shown in Table 2.


\textbf{Weakness 3.b Lower cost for memory and data in the search}

Besides the training time on GPU to finish the search, our method achieves a better performance with less memory and data. (a) Compared to LLM-Pruner, which identifies weight importance using backward passes, our method relies solely on inference. This significantly reduces GPU memory consumption, enhancing efficiency. (b) Compared to the SliceGPT, it requires 1024 data samples for calibration. Our method requires significantly fewer calibration samples (128) for weight optimization after the search, leading to better performance on  various datasets.




\textbf{Weakness 4. Quantization}

Quantization methods are not direct competitors but rather complementary to our search approach. Existing quantization methods can be applied to the subnets identified by our method, further enhancing acceleration through integer matrix multiplications. In practice, quantization methods require specialized computation kernels to handle integer matrix multiplications, which can introduce additional computational overhead and complexity in implementation, particularly during inference. This can pose challenges when deploying quantized models on diverse hardware platforms which may not support the quantized model. Our approach, on the other hand, maintains the original computation framework of LLMs, without the need for additional operations or specialized implementations.

Regarding the performance hit, we would like to clarify that the results in Table 7 were generated with a sequence length of 128, rather than 2048, for sequence length ablation study. Given that the dense LLaMA-7B model achieves the perplexity of 12.62 at 128 sequence length, our method, with a 90\% ratio, results in the perplexity of 13.40. This indicates a relatively small performance gap. With a larger sequence length such as 2048, the performance of all methods can be better and we can still achieve the best performance as shown in Table 2 and 3. 







\textbf{Question 1. Search cost and model size}

% pu:
% For the search cost, it usually takes only 20 epochs for the convergence, and more epochs beyond 20 lead to marginal improvements (see Figure 5). For LLaMA-7B, we run 50 epochs (5 hours) for better results. Thus, 20 epochs only cost 2 hours. For LLaMA-65B, we only adopt 20 epochs to get the subnets, which takes 5 hours. Larger models usually require more time for search, but the search can still be finished within 5 hours. 
% pu:
% For LLM-Pruner, it is very difficult to scale to larger models such as LLaMA-30B and LLaMA-65B, as it requires the backward propagation to compute the gradients for  identifying the weight importance, incurring much larger memory and complexity cost. It only has the results for 7B models (such as LLaMA-7B, and Vicuna-7B) and LLaMA-13B. The 7B models require 3 hours to finish the compression. 
% pu:
% For SliceGPT, it requires 5 hours to finish the pruning and fine-tuning of LLaMA-2 70B, which is similar to ours with 5 hours of search for LLaMA-65B. SliceGPT relies on PCA (Principal Component Analysis) to identify and remove less significant weights, which computes the eigenvectors and eigenvalues of the covariance matrix of the signal matrix. For large models, this step is computationally demanding and time-consuming because it requires processing a substantial amount of data to compute these matrices accurately. Besides, this work notes that using double precision for eigenvector calculations in PCA is necessary to avoid numerical errors that can degrade performance. This choice further increases the computational load and time required for pruning. It is data hungry and requires to use much more calibration samples (1024) while our method only uses 128 samples.

We discuss the search cost in detail at the global rebuttal. For LLaMA-7B, we still can achieve better performance than other methods when searching only with 20 epochs within 2 hours. For LLaMA-65B, we only adopt 20 epochs to get the subnets, which takes 5 hours.



\textbf{Question 2. Search cost with 5 hours}

% pu:
% The search cost is set to 5 hours empirically. We can reduce the search cost with comparable performance (still better than all baselines). As we mentioned above, for LLaMA-7B on one A100 GPU, it takes 5 hours for 50 epochs during the search process, and the search converges at 20 epochs as demonstrated in Figure 5, which only takes 2 hours. With only 20 epochs of search, the perplexity for LLaMA-7B with 10\% and 20\% sparsity on WikiText2 are 6.23 and 7.21, which are still better than all baselines in Table 2. Besides, for large models such as LLaMA-65B, we only adopt 20 epochs for faster search, which takes 5 hours. 

As we mentioned in global rebuttal, for LLaMA-7B on one A100 GPU, it takes 5 hours for 50 epochs during the search process, and the search converges at 20 epochs as demonstrated in Figure 5, which only takes 2 hours and achieves better performance than other methods. Besides, for large models such as LLaMA-65B, we only adopt 20 epochs for faster search, which takes 5 hours. 









% \textbf{Response to Reviewer Qp2U}
\textcolor{blue}{Response to Reviewer Qp2U}

% For question:

\textbf{Question 1. Comparison with SparseGPT} 

The pruning or search granularity of our method and SparseGPT are different, thus they should not be directly compared. Our method searches smaller compact models, which is more like the structural pruning method to remove rows and columns of weight matrices. Different from our structure search, SparseGPT is an irregular pruning method to remove weights without strong constraints (such as, the removed weights should be in the same rows or columns). Thus in the experiments, we compare with other structure pruning methods such as SliceGPT and FLAP, without comparing to SpareGPT. Furthermore, the baseline SliceGPT already provides certain comparisons with SparseGPT, as shown in Table 1 of SliceGPT. As mentioned above, it is hard to make a fair comparison between structure and irregular pruning. In Table 1 of SliceGPT, the sparsity of SparseGPT is 50\%, while the sparsity of SliceGPT is 25\% or 30\%. The results in their Table 1 can serve as a reference, and our method can outperform SliceGPT non-marginally.   











\textcolor{blue}{Response to Reviewer Xurt}

\textbf{Weakness 1. Search cost}

%pu:
% We can reduce the search cost with similar performance. For LLaMA-7B on one A100 (40G) GPU, it takes 5 hours for 50 epochs during the search. As shown in Figure 5 for convergence analysis, our method converges at 20 epochs, and more epochs do not result in significant improvements. We can reduce our search cost by only training 20 epochs, which just takes about 2 hours. Note that with 20 epochs, we can still achieve  6.23 and 7.21 perplexity on WikiText2 under 90\% and 80\% inheriting ratios, respectively, for LLaMA-7B, which are better than all baselines shown in Table 2. We can still perform better with reduced search cost. Besides, for large models such as LLaMA-65B, we only adopt 20 epochs for faster search, which takes 5 hours. 
%pu:
% Furthermore, our search cost is not significantly larger than baselines. As discussed in their original papers, LLM-Pruner requires 3 hours for the compression of LLaMA-7B. For SliceGPT, all LLaMA-2 , OPT and Phi-2 models can be sliced in 1 to 3 hours. With recovery fine-tuning, it compresses all LLMs in 1 to 5 hours in total. We can see that our search cost is similar to the baselines.  

As we discussed in the global rebuttal, we can reduce the search epoch from 50 to 20 for LLaMA-7B, which costs 2 hours and can still achieve better performance than other methods. For LLaMA-65B model, we only adopt 20 epochs for search, which costs 5 hours. Besides, compare to other methods, our search cost is similar to those baselines.







\textbf{Weakness 2. Post training performance}

To improve the performance, we adopt an efficient reformation method in Section 3.4 without the need of expensive training or finetuning. As shown in our Figure 6, our reformation can significantly improve the perplexity within a few minutes. We highlight that without training or finetuning, our method already outperforms baselines which are based on recovery training, such as LLM-Pruner and SliceGPT, as shown in our experimental results and Table 8 provided in global rebuttal.

To further evaluate our performance with continual training, we train our searched compact models with LoRA following the same setting of recovery training in LLM-Pruner, which can be finished within another 3 hours for LLaMA-7B. The results are demonstrated in Table 8 provided in global rebuttal. With recovery training, our method can further improve the perplexity and accuracy performance. For more sparse models (50\% inheriting ratio) suffering from more significant accuracy loss, recovery training can lead to larger improvements.  

Recovery training can further improve the accuracy, requiring more data and computations. Different from recovery training,  our reformation can efficiently and effectively lead to better performance than the baselines, with little data and computations. We agree that it is an attractive topic to investigate the pruned model performance with sufficient training. But for LLMs, it is still an open question how to define sufficient training, in terms of model architecture, data quality, data amount, GPUs, and so on. We leave this as our future research.





\textbf{Question 1. Mask sharing}

% pu:
% The layers in the same module of each block share the same mask, but different modules of different blocks do not share masks. To ensure the aligned internal computations, each attention block (i.e., one layer of LLaMA model) has two masks corresponding to its self-attention module and MLP module, respectively. Different attention blocks do not share masks, and they have their own masks, which are not necessarily the same. We believe the reviewer’s understanding is correct. For each block, we follow our mask sharing method in Line 139~149 to find its masks, and different blocks can have different masks. 

%The mask is shared for the query, key, and value within a single self-attention module, as well as for the up, gate, and down within a single MLP module, rather than being shared across different blocks.
%We discuss the mask sharing in detail at the global rebuttal upside.


The weights in the same module of each block share the same mask, but  different blocks do not share masks. Each block has its own masks, which are not shared with other blocks. The reviewer’s understanding is correct.  We discuss the mask sharing in detail in  the global rebuttal. Line 141 shows that there are two mask for each block, meaning there will be $2k$ masks for $k$ blocks, as the masks of different blocks are not shared.   


\textbf{Question 2. Fine-tuned compressed model compared to LLM-Pruner}

We show the results compared to the fine-tuned LLM-Pruner in Table 8 provided in global rebuttal. Results show that our method can perform better than LLM-Pruner even without finetuning.










\textcolor{blue}{Response to Reviewer BTSA}


\textbf{Weakness 1. Potential biased evaluation}

To mitigate the potential biased evaluation problem, we do not use the data from specific downstream tasks (QA datasets such as MMLU or ARC). Instead,  for our candidate evaluation and reformation, we use the general dataset WikiText2, which represents generic verified and featured articles on Wikipedia and makes sure that our experiments remain actually zero-shot since no task-specific downstream data is seen during our search. As the model never sees any downstream data  (so that it does not know how to be biased), it incurs less biased evaluation for downstream tasks. 
This setting is consistent with previous works such as FLAP and SliceGPT. 



To ensure a fair comparison, we use the same calibration dataset (i.e. WikiText2) for all methods including the baselines. We believe our evaluation is fair and comprehensive. Our method can achieve a better performance on language modeling and QA datasets. 
Furthermore,  FLAP investigates the performance with different  calibration datasets (see Appendix C.3 and  Table 7 of FLAP). It observes that C4 or WikiText2 as the calibration data, results in a fluctuation of about ±1\% in average accuracy for   zero-shot tasks, which is not significant. 







\textbf{Weakness 2. MMLU performance}

To make a fair comparison, we follow the setting in existing works (such as FLAP and SliceGPT) to use the data from WikiText2 for the candidate evaluation. Besides, it is super efficient to compute the perplexity of a few samples compared with testing the accuracy on the whole test set.

Following the suggestion, we demonstrate the performance on MMLU for our method and the baseline FLAP in Table 9 below. Our method can outperform the baseline in terms of accuracy on MMLU. 

As we mentioned in our response to Weakness 1, we use the  general dataset WikiText2 for candidate evaluation, which represents generic text data from Wikipedia and makes sure that our experiments remain actually zero-shot since no task-specific downstream data is seen during our search. Thus, our model is less biased for different downstream tasks. 

% -------------------- table 9 markdown ----------------
% Table 9

% | Inheriting Ratios | LLaMA-7B FLAP | LLaMA-7B Ours | LLaMA-13B FLAP | LLaMA-13B Ours | LLaMA-30B FLAP | LLaMA-30B Ours |
% |-------------------|---------------|---------------|----------------|----------------|----------------|----------------|
% | 100%              | 34.9          | 34.9          | 46.9           | 46.9           | 58.2           | 58.2           |
% | 90%               | 31.3          | **31.6**      | 40.3           | **40.3**       | 52.8           | **52.9**       |
% | 80%               | 29.1          | **29.2**      | 35.7           | **36.2**       | 47.3           | **47.6**       |
% | 70%               | 26.8          | **27.3**      | 33.4           | **33.7**       | 41.5           | **42.4**       |
% | 60%               | 25.9          | **26.3**      | 28.4           | **29.5**       | 36.1           | **37.4**       |
% | 50%               | 24.2          | **25.1**      | 27.9           | **29.1**       | 34.5           | **35.1**       |

% -------------------- table 9 markdown ----------------





\textbf{Weakness 3. QA performance in Table 5}

Following the suggestion, we further provide the results on the common sense reasoning datasets for the 50\% inheriting ratio in Table 8 provided in global rebuttal.
As observed, our method can lead to lower perplexity and higher downstream evaluation accuracy performance. 





\textbf{Weakness 4. Speed evaluation}

Thanks for the suggestion. For the generation speed test, we feed  sentences consisting of 64 tokens into the model and adopt float16 with KV cache. The flash attention is not activated. Our results in Figure 7 demonstrate that our smaller models lead to practical inference acceleration. We agree that the inference speed may be different under different evaluation settings. Following the suggestion, we further show the computation cost in GMACs in Table 10 below.


% ----------------Table 10 markdown ----------------
% Table 10 

% | Inheriting Ratio        | 100%  | 90%   | 80%   | 70%   | 60%   | 50%   |
% |-------------------------|-------|-------|-------|-------|-------|-------|
% | Computation Cost (GMACs)| 424.02| 377.89| 333.49| 293.29| 249.28| 211.88|
% ----------------Table 10 markdown ----------------








\textbf{Question 1. Writing issues}

Yes, the reviewer’s understanding is correct, and "inheriting ratio" = 1 - "sparsity". We provide an explanation for the inheriting ratio in Line 116-117. 



\textbf{Question 2. Annotation}

Thanks, we will add the annotation.








\textbf{Question 3. Clarification}

M denotes the number of heads in attention, P denotes the number of channels in MLP (intermediate size). Masks are binary, it should be {0,1} rather than R.  We will make it more clear in the revision

\textbf{Question 3.a Mask sharing}
%pu:
% As discussed in Line 124-128, the model has multiple attention blocks (i.e., layers of LLaMA model). Each block has two modules, the self-attention module and MLP module. Each module contains multiple layers, such as the query, key, value in the self-attention module (Line 124-128). Mask sharing means that different layers in the same module share the same mask. However, modules inside different blocks do not necessarily share the same mask. Each attention block has two masks corresponding to its self-attention module and MLP module, respectively. Different attention blocks do not share masks, and they have their own masks, which are not necessarily the same. Just as the reviewer mentioned, Figure 2 middle shows that different attention blocks can have different masks/sparsity. Note that the concepts of blocks and layers are different and they do not mean the same thing in our paper.
%pu:
% Initially, different masks have the same inheriting ratios. But the masks can still be different although their sparsity are the same. After we begin our search, the inheriting ratios of different masks  can be different, although they start from the same value.

The mask is shared for the query, key, and value within a single self-attention module, as well as for the up, gate, and down within a single MLP module, rather than being shared across different blocks.
We discuss the mask sharing in detail in  the above global rebuttal.

\textbf{Question 3.b Align internal computations}

As discussed in Line 141-142, for multiple layers inside each module (self-attention or MLP), they have to use the same mask to ensure the aligned internal computations. For example, if the query and key have different masks and thus different/unaligned dimensions, they can not be multiplied elementwise and  the attention operation can not be correctly performed. In Appendix A, we demonstrate the mechanism for the self-attention and MLP modules, highlighting that the layers inside the same module need to share the same mask to ensure successful computations. But layers in different modules or blocks do not need to share the same mask. We are sorry for any confusion and will make this more clear in the revision. 

\textbf{Question 3.c Joint optimization of masks}

They are jointly optimized to determine the initial masks as discussed in Line 147-149. Later during our search, all masks are also jointly optimized to satisfy the parameter count constraint.














\textbf{Question 4. Gamma}

$\gamma_{attn}^i$ denotes the inheriting ratio for the $i^{th}$ head in attention. Each attention module can have multiple heads. Thus the inheriting ratio for the attention module is a collection from multiple heads as the inheriting ratio for each head can be different. $\gamma_{mlp}$ denotes the inheriting ratio of the MLP module. It does not have the concepts of multiple heads like the attention module and we just have one single ratio for the whole MLP.






\textbf{Limitation: Search cost}
%pu:
% We can reduce the search cost with similar performance. For LLaMA-7B on one A100 (40G) GPU, it takes 5 hours for 50 epochs during the search. As shown in Figure 5 for convergence analysis, our method converges at about 20 epochs, and more epochs lead to marginal improvements. We can reduce our search cost by only training 20 epochs, which just takes about 2 hours. Note that with 20 epochs, we can still achieve  6.23 and 7.21 perplexity on WikiText2 under 90\% and 80\% inheriting ratios, respectively, for LLaMA-7B, which are better than all baselines shown in Table 2. We can still perform better with reduced search cost. Besides, for large models such as LLaMA-65B, we only adopt 20 epochs for faster search, which takes 5 hours. 
%pu:
% Furthermore, our search cost is not significantly larger than baselines. As discussed in their original papers, LLM-Pruner requires 3 hours for the compression of LLaMA-7B. For SliceGPT, all LLaMA-2 , OPT and Phi-2 models can be sliced in 1 to 3 hours. With recovery fine-tuning, it compresses all LLMs in 1 to 5 hours in total. We can see that our search cost is similar to the baselines. 


As we discussed in global rebuttal, the search cost can be reduced to 20 epochs within 2 hours and is similar to those baselines.






\clearpage

\input{tables/results_compare_to_finetuned_llmpruner}



\input{tables/results_mmlu_gsm8k}


\input{tables/results_computation_cost_llama_7b}







==> tables/results_compare_to_finetuned_llmpruner.tex <==



\begin{table}[t]
% \vspace{-0.5cm}
\centering
\caption{
Comparison to the LoRA fine-tuned compressed LLaMA-7B model.
}
% \vspace{-0.25cm}
\label{tab:compare_to_finetuned_model}
\resizebox{1.0\linewidth}{!}{
\begin{tabular}{c|c|cc|ccccccc|c}

\toprule
% Method & Sparsity & Wiki $\downarrow$    & PTB $\downarrow$            & BoolQ & PIQA  & HellaSwag & WinoGrande & ARC-e          & ARC-c & OBQA & Average  $\uparrow$       \\
\multirow{2}{*}{Method} & Inheriting & Wiki    & PTB     & \multirow{2}{*}{BoolQ} & \multirow{2}{*}{PIQA}  & Hella & Wino & \multirow{2}{*}{ARC-e}          & \multirow{2}{*}{ARC-c}  & \multirow{2}{*}{OBQA}  & Average         \\
 & Ratio & PPL$\downarrow$ & PPL$\downarrow$ & & & Swag & Grande & & & & Acc.$\uparrow$ \\
% \midrule
\toprule
% LLM-Pruner       &   80\%   & 10.73         & 59.73         & 57.06 & 75.68 & 66.80            & 59.83      & 60.94          & 36.52       & 40.00   & 56.69           \\
LLM-Pruner        &  80\%    & 11.97         & 55.68         & 59.39 & 75.57 & 65.34           & 61.33      & 59.18          & 37.12       & 39.80 & 56.82           \\
LLM-Pruner (LoRA)      &   80\%   & 8.41         & 41.78         & 67.78 & 76.36 & 68.14            & 64.32      & 63.41          & 36.87       & 40.10   &    59.57        \\
\midrule
Ours            & 80\%     & \textbf{6.89} & \textbf{36.06} & 70.98 & 74.92 & 67.29           & 64.64      & 64.23          & 36.52       & 39.40 & \textbf{59.71}  \\
\midrule
Ours (LoRA)           & 80\%     & 6.57 & 34.32 & 71.19 & 75.01 & 68.43           & 64.12      & 63.88          & 35.44       & 40.03 & 59.73  \\
% \midrule
\bottomrule
\toprule
LLM-Pruner       &   50\%   & 126.02         & 460.71         & 51.97 & 60.23 & 35.89            & 49.07      & 32.76          & 25.67       & 34.91   & 41.50           \\
LLM-Pruner (LoRA)      &   50\%   & 51.56         & 198.76       &  60.98 &	69.12	&47.83	&55.78	&46.92	&28.56	&35.64	&49.26\\
\midrule
Ours            & 50\%     & \textbf{15.48} & \textbf{117.06} & 61.27 & 69.13 & 51.18           & 57.78      & 52.16          & 29.34       & 35.45 & \textbf{50.79}  \\
\midrule
Ours (LoRA)           & 50\%     & 11.34 & 83.48 & 63.49 & 73.03 & 56.93           & 59.21      & 48.87          & 36.12       & 36.23 &  53.41  \\
\bottomrule
\end{tabular}
}
% \vspace{-0.4cm}
\end{table}



==> tables/results_computation_cost_llama_7b.tex <==





\begin{table}[]
\centering
\caption{
Computation cost of LLaMA-7B model with different inheriting ratios.
}
\resizebox{0.7\linewidth}{!}{
\begin{tabular}{c|ccccc c}
\toprule
Inheriting Ratio & 100\% & 90\% & 80\% & 70\% & 60\% & 50\%\\
Computation Cost (GMACs) & 424.02 & 377.89 & 333.49 & 293.29 & 249.28 & 211.88 \\
\bottomrule
\end{tabular}
}
\label{tab:computation_cost}
\end{table}






==> tables/results_llama7b_13b_larger_sparsity.tex <==



% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[h]
\caption{
Comparison for larger sparsity on LLaMA-7B and LLaMA-13B.
% Results are evaluated on the WikiText2 and PTB datasets with the 2048 sequence length.
% The same 128 samples from the WikiText2 training dataset are used to calibrate SliceGPT, FLAP, and our method.
}
\centering
\resizebox{0.74\linewidth}{!}{
\begin{tabular}{c|c|ccc|ccc}
\toprule
\multicolumn{2}{c|}{Model}                   & \multicolumn{3}{c|}{LLaMA-7B}                      & \multicolumn{3}{c}{LLaMA-13B}                    \\
\midrule
Dataset                    & Sparsity       & 30\%           & 40\%           & 50\%            & 30\%           & 40\%           & 50\%           \\
\toprule
\multirow{4}{*}{WikiText2} & LLM-Pruner(e1) & 18.58          & 38.27          & 125.96          & 22.36          & 66.38          & 3827.63        \\
                           & SliceGPT       & 15.95          & 279.52         & 1830.43         & 9.79           & 13.21          & 19.950         \\
                           & FLAP           & 9.177          & 12.34          & 21.89           & 6.97           & 8.67           & 12.88          \\
                           & Ours           & \textbf{8.28}  & \textbf{10.21} & \textbf{15.48}  & \textbf{6.67}  & \textbf{8.00}  & \textbf{10.44} \\
                           \midrule
\multirow{4}{*}{PTB}       & LLM-Pruner(e1) & 93.24          & 238.09         & 460.73          & 112.03         & 278.36         & 1287.11        \\
                           & SliceGPT       & 583.58         & 5186.06        & 15333.66        & 167.27         & 247.71         & 408.68         \\
                           & FLAP           & 47.35          & 65.55          & 135.84          & 27.38          & 35.91          & 53.54          \\
                           & Ours           & \textbf{45.26} & \textbf{62.07} & \textbf{117.06} & \textbf{26.37} & \textbf{33.23} & \textbf{45.73} \\
\bottomrule
\end{tabular}
}
\end{table}



==> tables/results_mmlu_gsm8k.tex <==



% \begin{table}[]
% \centering
% \caption{
% Results of LLaMA models on MMLU datasets.
% }
% \resizebox{0.5\linewidth}{!}{
% \begin{tabular}{c|c|c|c}
% \toprule
% Inheriting Ratio & LLaMA-7B & LLaMA-13B & LLaMA-30B \\
% \midrule
% 100\%    & 34.9                    & 46.9                   & 58.2                  \\
% \midrule
% 90\%     & 31.6                   & 40.3                    & 52.9               \\
% 80\%     & 29.2                   & 36.2                & 47.6            \\
% 70\%     & 27.3                  & 33.7                   & 42.4                 \\
% 60\%     & 26.3                  & 29.5                   & 37.4                \\
% 50\%     & 25.1                  & 29.1                  & 35.1             \\
% \bottomrule
% \end{tabular}
% }
% \label{tab:mmlu_gsm8k}
% \end{table}


\begin{table}[]
\centering
\caption{
Results of LLaMA models on MMLU datasets.
}
\resizebox{0.6\linewidth}{!}{
\begin{tabular}{c|cc|cc|cc}
\toprule
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Inheriting\\ Ratios\end{tabular}} & \multicolumn{2}{c|}{LLaMA-7B} & \multicolumn{2}{c|}{LLaMA-13B} & \multicolumn{2}{c}{LLaMA-30B} \\ \cline{2-7}
                                                                             & FLAP          & Ours         & FLAP          & Ours          & FLAP          & Ours          \\
                                                                             \midrule
100\%                                                                        & \multicolumn{2}{c|}{34.9}     & \multicolumn{2}{c|}{46.9}      & \multicolumn{2}{c}{58.2}      \\
\midrule
90\%                                                                         & 31.3     & \textbf{31.6}     & 40.3      & \textbf{40.3}     & 52.8      & \textbf{52.9}     \\
80\%                                                                         & 29.1     & \textbf{29.2}     & 35.7      & \textbf{36.2}     & 47.3      & \textbf{47.6}     \\
70\%                                                                         & 26.8     & \textbf{27.3}     & 33.4      & \textbf{33.7}     & 41.5      & \textbf{42.4}     \\
60\%                                                                         & 25.9     & \textbf{26.3}     & 28.4      & \textbf{29.5}     & 36.1      & \textbf{37.4}     \\
50\%                                                                         & 24.2     & \textbf{25.1}     & 27.9      & \textbf{29.1}     & 34.5      & \textbf{35.1}    \\
\bottomrule
\end{tabular}
}
\label{tab:mmlu_gsm8k}
\end{table}


==> tables/results_opt.tex <==


\begin{table}[h]
\caption{
Results of the compressed OPT models.
}
\centering
\resizebox{1\linewidth}{!}{
\begin{tabular}{c|c|cc|cc|cc}
\toprule
\multicolumn{2}{c}{Sparsity} & \multicolumn{2}{c}{10\%}        & \multicolumn{2}{c}{20\%}        & \multicolumn{2}{c}{30\%}         \\
\toprule
Size        & Method         & Wiki           & PTB            & Wiki           & PTB            & Wiki           & PTB             \\
\toprule
125M        & SliceGPT       & 35.31          & 75.59          & 54.88          & 149.17         & 84.16          & 245.18          \\
125M        & Ours           & \textbf{30.97} & \textbf{40.14} & \textbf{44.12} & \textbf{66.55} & \textbf{80.84} & \textbf{124.27} \\
\midrule
1.3B        & SliceGPT       & 16.74          & 35.31          & 20.17          & 61.30          & 28.53          & 113.42          \\
1.3B        & Ours           & \textbf{15.51} & \textbf{20.19} & \textbf{19.23} & \textbf{32.81} & \textbf{26.82} & \textbf{69.42}  \\
\midrule
2.7B        & SliceGPT       & 14.10          & 37.01          & 16.81          & 65.09          & 24.12          & 132.13          \\
2.7B        & Ours           & \textbf{13.32} & \textbf{17.24} & \textbf{16.44} & \textbf{23.66} & \textbf{23.48} & \textbf{58.46} \\
\bottomrule
\end{tabular}
}
\end{table}



==> tables/search_space_llama.tex <==



% % \begin{wraptable}{r}{0.5\textwidth}
% \begin{table}[]

% % \vspace{-0.5cm}
% \centering
% \resizebox{1.0\linewidth}{!}{

% \begin{tabular}{c|ccc |ccc |ccc   |   ccc| ccc| ccc| ccc}
% \toprule
% \multicolumn{1}{c|}{Model} & \multicolumn{9}{c|}{OPT Family} & \multicolumn{12}{c}{LLaMA Family}  \\
% \midrule
%  Scale   & \multicolumn{3}{c|}{OPT-125M}  & \multicolumn{3}{c|}{OPT-1.3B}   & \multicolumn{3}{c|}{OPT-2.7B}       & \multicolumn{3}{c|}{LLaMA-7B} & \multicolumn{3}{c|}{LLaMA-13B} & \multicolumn{3}{l|}{LLaMA-30B} & \multicolumn{3}{l}{LLaMA-65B}  \\
% \midrule

%  Sparsity   & $d$ & $\rho_{attn}$ & $\rho_{mlp}$ & $d$ & $\rho_{attn}$ & $\rho_{mlp}$   & $d$ & $\rho_{attn}$ & $\rho_{mlp}$       & $d$ & $\rho_{attn}$ & $\rho_{mlp}$ & $d$ & $\rho_{attn}$ & $\rho_{mlp}$ & $d$ & $\rho_{attn}$ & $\rho_{mlp}$ & $d$ & $\rho_{attn}$ & $\rho_{mlp}$ \\
% \midrule

% 10\% & (10,12,1) \\

% 20\% &  \\

% 30\% &  \\

% 40\% &  \\

% 50\% &  \\

% \bottomrule
% \end{tabular}

% }
% \caption{123}
% \label{tab:search_space}
% \end{table}
% % \vspace{-0.5cm}
% % \end{wraptable}





% \begin{wraptable}{r}{0.5\textwidth}
\begin{table}[]

% \vspace{-0.5cm}
\centering
\resizebox{1.0\linewidth}{!}{

\begin{tabular}{c|cccc| cc}
\toprule
Space & \multicolumn{4}{c|}{Model Depth} & \multicolumn{2}{c}{Sparsity Ratio}  \\
\midrule
 Sparsity   &  LLaMA-7B & LLaMA-13B & LLaMA-30B & LLaMA-65B & $\rho_{attn}$ & $\rho_{mlp}$   \\
\midrule


10\% & [32,32,1] & [40,40,1] & [60,60,1] & [80,80,1] \\

20\% & [32,32,1] & [40,40,1] & [60,60,1] & [80,80,1]  \\

30\% & [30,32,1] & [36,40,1] & [56,60,1] & [76,80,1]  \\

40\% & [28,32,1] & [32,40,1] & [52,60,1] & [72,80,1]  \\

50\% & [28,32,1] & [32,40,1] & [52,60,1] & [72,80,1]  \\

\bottomrule
\end{tabular}

}
\caption{123}
\label{tab:search_space}
\end{table}
% \vspace{-0.5cm}
% \end{wraptable}














